Trajectory Control for Differential Drive Mobile Manipulators

Mobile manipulator systems are comprised of a mobile platform with one or more manipulators and are of great interest in a number of applications such as indoor warehouses, mining, construction, forestry etc. We present an approach for computing actuator commands for such systems so that they can follow desired end-effector and platform trajectories without the violation of the nonholonomic constraints of the system in an indoor warehouse environment. We work with the Fetch robot which consists of a 7-DOF manipulator with a differential drive mobile base to validate our method. The major contributions of our project are, writing the dynamics of the system, Trajectory planning for the manipulator and the mobile base, state machine for the pick and place task and the inverse kinematics of the manipulator. Our results indicate that we are able to successfully implement trajectory control on the mobile base and the manipulator of the Fetch robot.

==> bib1.tex <==
@article{correll2016lessons,
  title={Lessons from the amazon picking challenge},
  author={Correll, Nikolaus and Bekris, Kostas E and Berenson, Dmitry and Brock, Oliver and Causo, Albert and Hauser, Kris and Okada, Kei and Rodriguez, Alberto and Romano, Joseph M and Wurman, Peter R},
  journal={arXiv preprint arXiv:1601.05484},
  year={2016}
}
